The highly polarized open cluster Trumpler 27

We have carried out multicolor linear polarimetry (UBVRI) of the brightest stars in the area of the open cluster Trumpler 27. Our data show a high level of polarization in the stellar light with a considerable dispersion, from $P = 4%$ to $P = 9.5%$. The polarization vectors of the cluster members appear to be aligned. Foreground polarization was estimated from the data of some non-member objects, for which two different components were resolved: the first one associated with a dust cloud close to the Sun producing $P_{\lambda max}=1.3%$ and $\theta=146$ degrees, and a second component, the main source of polarization for the cluster members, originated in another dust cloud, which polarizes the light in the direction of $\theta= 29.5$ degrees. From a detailed analysis, we found that the two components have associated values $E_{B-V} < 0.45 $ for the first one, and $E_{B-V} > 0.75$ for the other. Due the difference in the orientation of both polarization vectors, almost 90 degrees (180 degrees at the Stokes representation), the first cloud ($\theta \sim 146$ degrees) depolarize the light strongly polarized by the second one ($\theta \sim 29.5$ degrees).

==> Feinstein.tab1.tex <==


%\documentstyle[12pt,aj_pt4]{article}
%\begin{document}
%\pagestyle{empty}


\tablewidth{300pt}
\makeatletter
\def\jnl@aj{AJ}
\ifx\revtex@jnl\jnl@aj\let\tablebreak=\nl\fi



%\addtocounter{table}{+3}%
\begin{planotable}{lcc}
\tablecaption {Polarimetric Observations of stars in Tr 27}
\tablehead{
  \colhead{Filter} &
  \colhead{ $P_{\lambda} \pm \epsilon_{P}$} &
  \colhead{$\theta_{\lambda} \pm \epsilon_{\theta}$ } \\ 
     \colhead { } &
     \colhead{$\%$} &
     \colhead{(deg)} 
}
\startdata
Star 1 & &   \nl
B & 6.65 $\pm$ 0.09 & 32.0 $\pm$ 0.4 \nl
V & 6.47 $\pm$ 0.08 & 37.2 $\pm$ 0.4 \nl
R & 5.63 $\pm$ 0.03 & 43.8 $\pm$ 0.1 \nl
I & 5.37 $\pm$ 0.07 & 40.2 $\pm$ 0.4 \nl
Star 2 & &   \nl
U & 5.65 $\pm$ 0.15 & 24.1 $\pm$ 0.8 \nl
B & 6.53 $\pm$ 0.02 & 21.7 $\pm$ 0.1 \nl
V & 6.75 $\pm$ 0.02 & 22.2 $\pm$ 0.1 \nl
R & 6.25 $\pm$ 0.01 & 21.9 $\pm$ 0.1 \nl
I & 5.67 $\pm$ 0.01 & 22.4 $\pm$ 0.1 \nl
Star 4 & &   \nl
B & 1.04 $\pm$ 0.26 & 146.4 $\pm$ 6.9 \nl
V & 1.48 $\pm$ 0.20 & 138.5 $\pm$ 3.8 \nl
R & 1.47 $\pm$ 0.15 & 140.1 $\pm$ 2.9 \nl
I & 1.55 $\pm$ 0.29 & 125.5 $\pm$ 5.4 \nl
Star 5 & &   \nl
U & 4.18 $\pm$ 0.62 & 38.8 $\pm$ 4.2 \nl
B & 1.63 $\pm$ 0.66 & 60.8 $\pm$ 11.1 \nl
V & 1.00 $\pm$ 0.76 & 46.8 $\pm$ 18.7 \nl
Star 6 & &   \nl
B & 1.80 $\pm$ 0.28 & 140.3 $\pm$ 4.3 \nl
V & 1.48 $\pm$ 0.08 & 142.1 $\pm$ 1.6 \nl
R & 1.51 $\pm$ 0.08 & 142.2 $\pm$ 1.4 \nl
I & 1.18 $\pm$ 0.13 & 140.9 $\pm$ 3.1 \nl
Star 8 & &   \nl
U & 7.32 $\pm$ 0.57 & 37.3 $\pm$ 2.2 \nl
B & 6.74 $\pm$ 0.40 & 38.3 $\pm$ 1.7 \nl
V & 7.72 $\pm$ 0.26 & 38.5 $\pm$ 1.0 \nl
R & 7.16 $\pm$ 0.18 & 41.2 $\pm$ 0.7 \nl
I & 6.32 $\pm$ 0.17 & 41.6 $\pm$ 0.8 \nl
Star 10 & &   \nl
U & 7.28 $\pm$ 0.65 & 30.3 $\pm$ 2.5 \nl
B & 8.05 $\pm$ 0.44 & 32.7 $\pm$ 1.6 \nl
V & 7.70 $\pm$ 0.29 & 34.4 $\pm$ 1.1 \nl
R & 6.79 $\pm$ 0.17 & 33.8 $\pm$ 0.7 \nl
I & 5.85 $\pm$ 0.15 & 35.5 $\pm$ 0.7 \nl
Star 11 & &   \nl
U & 3.06 $\pm$ 0.35 & 33.5 $\pm$ 3.3 \nl
B & 3.73 $\pm$ 0.29 & 36.2 $\pm$ 2.2 \nl
V & 4.32 $\pm$ 0.29 & 37.2 $\pm$ 1.9 \nl
R & 4.58 $\pm$ 0.15 & 37.6 $\pm$ 0.9 \nl
I & 4.21 $\pm$ 0.16 & 40.3 $\pm$ 1.1 \nl
Star 14 & &   \nl
V & 4.64 $\pm$ 0.04 & 29.1 $\pm$ 0.3 \nl
R & 4.24 $\pm$ 0.05 & 29.3 $\pm$ 0.4 \nl
I & 4.05 $\pm$ 0.05 & 29.7 $\pm$ 0.4 \nl
Star 16 & &   \nl
U & 4.10 $\pm$ 0.19 & 26.9 $\pm$ 1.3 \nl
B & 5.06 $\pm$ 0.01 & 28.7 $\pm$ 0.1 \nl
V & 5.35 $\pm$ 0.02 & 29.9 $\pm$ 0.1 \nl
R & 5.22 $\pm$ 0.02 & 31.4 $\pm$ 0.1 \nl
I & 4.72 $\pm$ 0.01 & 31.3 $\pm$ 0.1 \nl
Star 19 & &   \nl
U & 3.28 $\pm$ 0.48 & 26.7 $\pm$ 4.1 \nl
B & 3.51 $\pm$ 0.37 & 27.9 $\pm$ 3.0 \nl
V & 3.85 $\pm$ 0.32 & 29.7 $\pm$ 2.4 \nl
R & 3.44 $\pm$ 0.18 & 30.2 $\pm$ 1.5 \nl
I & 2.62 $\pm$ 0.21 & 33.9 $\pm$ 2.3 \nl
Star 21 & &   \nl
U & 3.47 $\pm$ 0.65 & 26.0 $\pm$ 5.3 \nl
B & 3.40 $\pm$ 0.48 & 25.3 $\pm$ 4.1 \nl
V & 3.58 $\pm$ 0.38 & 26.6 $\pm$ 3.0 \nl
R & 3.77 $\pm$ 0.16 & 26.2 $\pm$ 1.2 \nl
I & 3.00 $\pm$ 0.23 & 25.6 $\pm$ 2.2 \nl
Star 22 & &   \nl
U & 1.94 $\pm$ 0.55 & 150.7 $\pm$ 7.8 \nl
B & 1.23 $\pm$ 0.28 & 143.7 $\pm$ 6.3 \nl
V & 1.30 $\pm$ 0.08 & 151.9 $\pm$ 1.6 \nl
R & 1.31 $\pm$ 0.07 & 150.1 $\pm$ 1.6 \nl
I & 1.02 $\pm$ 0.15 & 144.4 $\pm$ 4.1 \nl
Star 23 & &   \nl
U & 8.03 $\pm$ 0.64 & 26.5 $\pm$ 2.3 \nl
B & 9.04 $\pm$ 0.10 & 27.5 $\pm$ 0.3 \nl
V & 9.56 $\pm$ 0.09 & 27.2 $\pm$ 0.3 \nl
R & 8.86 $\pm$ 0.03 & 27.7 $\pm$ 0.1 \nl
I & 7.91 $\pm$ 0.02 & 27.6 $\pm$ 0.1 \nl
Star 24 & &   \nl
U & 1.10 $\pm$ 0.16 & 152.0 $\pm$ 4.1 \nl
B & 1.21 $\pm$ 0.11 & 147.9 $\pm$ 2.6 \nl
V & 1.32 $\pm$ 0.10 & 148.5 $\pm$ 2.1 \nl
R & 1.32 $\pm$ 0.07 & 150.4 $\pm$ 1.5 \nl
I & 1.15 $\pm$ 0.09 & 148.7 $\pm$ 2.2 \nl
Star 25 & &   \nl
U & 7.74 $\pm$ 0.19 & 31.6 $\pm$ 0.7 \nl
B & 8.38 $\pm$ 0.03 & 30.8 $\pm$ 0.1 \nl
V & 9.24 $\pm$ 0.06 & 30.6 $\pm$ 0.2 \nl
R & 8.64 $\pm$ 0.03 & 30.1 $\pm$ 0.1 \nl
I & 7.98 $\pm$ 0.03 & 30.8 $\pm$ 0.1 \nl
Star 26 & &   \nl
V & 1.20 $\pm$ 0.07 & 151.5 $\pm$ 1.7 \nl
Star 27 & &   \nl
B & 7.71 $\pm$ 0.95 & 45.4 $\pm$ 3.5 \nl
V & 9.32 $\pm$ 0.41 & 42.7 $\pm$ 1.3 \nl
R & 9.31 $\pm$ 0.18 & 42.8 $\pm$ 0.6 \nl
I & 8.07 $\pm$ 0.24 & 42.6 $\pm$ 0.8 \nl
Star 28 & &   \nl
U & 4.06 $\pm$ 1.54 & 68.4 $\pm$ 10.4 \nl
B & 4.24 $\pm$ 1.01 & 29.5 $\pm$ 6.7 \nl
V & 5.10 $\pm$ 0.76 & 39.2 $\pm$ 4.3 \nl
R & 5.39 $\pm$ 0.24 & 35.3 $\pm$ 1.3 \nl
I & 4.84 $\pm$ 0.17 & 35.2 $\pm$ 1.0 \nl
Star 30 & &   \nl
U & 6.92 $\pm$ 1.35 & 24.4 $\pm$ 5.5 \nl
B & 7.77 $\pm$ 0.80 & 33.3 $\pm$ 2.9 \nl
V & 7.80 $\pm$ 0.55 & 32.4 $\pm$ 2.0 \nl
R & 7.23 $\pm$ 0.22 & 34.6 $\pm$ 0.9 \nl
I & 6.50 $\pm$ 0.34 & 35.3 $\pm$ 1.5 \nl
Star 32 & &   \nl
U & 4.26 $\pm$ 0.36 & 27.0 $\pm$ 2.4 \nl
B & 4.53 $\pm$ 0.38 & 28.0 $\pm$ 2.4 \nl
V & 4.54 $\pm$ 0.30 & 28.8 $\pm$ 1.9 \nl
R & 4.63 $\pm$ 0.12 & 29.2 $\pm$ 0.7 \nl
I & 3.64 $\pm$ 0.19 & 28.8 $\pm$ 1.5 \nl
Star 34 & &   \nl
U & 3.21 $\pm$ 0.41 & 23.8 $\pm$ 3.6 \nl
B & 4.09 $\pm$ 0.47 & 27.7 $\pm$ 3.2 \nl
V & 3.94 $\pm$ 0.30 & 25.2 $\pm$ 2.2 \nl
R & 4.07 $\pm$ 0.14 & 25.0 $\pm$ 1.0 \nl
I & 3.70 $\pm$ 0.27 & 25.0 $\pm$ 2.1 \nl
Star 43 & &   \nl
U & 5.79 $\pm$ 0.31 & 36.2 $\pm$ 1.5 \nl
B & 6.55 $\pm$ 0.15 & 34.0 $\pm$ 0.6 \nl
V & 6.67 $\pm$ 0.16 & 33.4 $\pm$ 0.7 \nl
R & 6.21 $\pm$ 0.15 & 35.3 $\pm$ 0.7 \nl
I & 5.47 $\pm$ 0.13 & 35.1 $\pm$ 0.7 \nl
Star 46 & &   \nl
B & 6.59 $\pm$ 0.05 & 28.9 $\pm$ 0.2 \nl
V & 6.88 $\pm$ 0.06 & 29.1 $\pm$ 0.2 \nl
R & 6.23 $\pm$ 0.05 & 29.8 $\pm$ 0.2 \nl
Star 102 & &   \nl
U & 5.51 $\pm$ 0.59 & 26.5 $\pm$ 3.1 \nl
B & 5.00 $\pm$ 0.29 & 23.0 $\pm$ 1.7 \nl
V & 5.03 $\pm$ 0.02 & 24.0 $\pm$ 0.1 \nl
R & 4.68 $\pm$ 0.01 & 24.0 $\pm$ 0.1 \nl
I & 4.18 $\pm$ 0.01 & 24.7 $\pm$ 0.1 \nl
Star 103 & &   \nl
U & 1.06 $\pm$ 0.22 & 11.9 $\pm$ 5.9 \nl
B & 1.181 $\pm$ 0.08 & 11.3 $\pm$ 0.1 \nl
V & 1.36 $\pm$ 0.06 & 9.9 $\pm$ 1.2 \nl
R & 1.82 $\pm$ 0.00 & 11.4 $\pm$ 0.1 \nl
I & 1.28 $\pm$ 0.11 & 11.6 $\pm$ 2.5 \nl
Star 104 & &   \nl
U & 2.86 $\pm$ 0.12 & 20.4 $\pm$ 1.2 \nl
B & 3.33 $\pm$ 0.12 & 18.1 $\pm$ 1.0 \nl
V & 3.40 $\pm$ 0.09 & 19.9 $\pm$ 0.7 \nl
R & 3.51 $\pm$ 0.08 & 19.1 $\pm$ 0.6 \nl
I & 3.13 $\pm$ 0.07 & 19.8 $\pm$ 0.6 \nl
Star 105 & &   \nl
U & 4.50 $\pm$ 0.47 & 53.5 $\pm$ 3.0 \nl
B & 4.82 $\pm$ 0.04 & 51.2 $\pm$ 0.3 \nl
V & 5.20 $\pm$ 0.04 & 49.1 $\pm$ 0.2 \nl
R & 5.20 $\pm$ 0.01 & 48.9 $\pm$ 0.1 \nl
I & 4.88 $\pm$ 0.02 & 48.4 $\pm$ 0.1 \nl
Star 106 & &   \nl
U & 2.97 $\pm$ 0.19 & 23.6 $\pm$ 1.8 \nl
B & 3.05 $\pm$ 0.03 & 21.4 $\pm$ 0.3 \nl
V & 3.40 $\pm$ 0.03 & 23.3 $\pm$ 0.3 \nl
R & 3.51 $\pm$ 0.01 & 22.9 $\pm$ 0.1 \nl
I & 3.47 $\pm$ 0.02 & 22.5 $\pm$ 0.2 \nl
Star 107 & &   \nl
U & 3.71 $\pm$ 0.19 & 24.2 $\pm$ 1.5 \nl
B & 3.98 $\pm$ 0.18 & 23.4 $\pm$ 1.3 \nl
V & 4.39 $\pm$ 0.20 & 24.0 $\pm$ 1.3 \nl
R & 4.24 $\pm$ 0.13 & 24.1 $\pm$ 0.9 \nl
I & 3.75 $\pm$ 0.18 & 23.7 $\pm$ 1.4 \nl
\enddata
\end{planotable}

%\end{document}


